DAGnosis: Localized Identification of Data Inconsistencies using Structures

Identification and appropriate handling of inconsistencies in data at deployment time is crucial to reliably use machine learning models. While recent data-centric methods are able to identify such inconsistencies with respect to the training set, they suffer from two key limitations: (1) suboptimality in settings where features exhibit statistical independencies, due to their usage of compressive representations and (2) lack of localization to pin-point why a sample might be flagged as inconsistent, which is important to guide future data collection. We solve these two fundamental limitations using directed acyclic graphs (DAGs) to encode the training set's features probability distribution and independencies as a structure. Our method, called DAGnosis, leverages these structural interactions to bring valuable and insightful data-centric conclusions. DAGnosis unlocks the localization of the causes of inconsistencies on a DAG, an aspect overlooked by previous approaches. Moreover, we show empirically that leveraging these interactions (1) leads to more accurate conclusions in detecting inconsistencies, as well as (2) provides more detailed insights into why some samples are flagged.

==> tables/adult_numbers.tex <==

\begin{table}[h]
\vspace{-10pt}
	\centering
	\caption{\textbf{Analysis of the features of flagged samples} We report the proportion of test samples which are flagged and have the attribute \textit{Sex = 0}, and the proportion of test samples which are flagged and have the attribute \textit{Sex = 1}. DAGnosis has an edge over Data-SUITE because it flags more inconsistent samples (\textit{Sex = 0}), while flagging a similar number of men. In the below, ``Sex=0'' indicates ${\lvert \mathcal{D}_{\mathrm{flagged, sex= 0}}^{(5)}  \rvert }/{\lvert \mathcal{D}_{\mathrm{test}}^{(5)} \rvert} $, and ``Sex=1'' indicates ${\lvert \mathcal{D}_{\mathrm{flagged, sex= 1}}^{(5)}  \rvert }/{\lvert \mathcal{D}_{\mathrm{test}}^{(5)} \rvert} $. DAGnosis is in \colorbox{green!10}{green}.}
	\vspace{0.2em}
	\label{tab:detection_adult}
	
	\begin{tabularx}{\linewidth}{r|C|C}
		\toprule
			 &   Sex=0 & Sex=1\\
        \toprule

        \textbf{\em Data-SUITE} & 0.08 & 0.040 \\
        \rowcolor{green!10}\textbf{\em DAGnosis (PC)} & 0.11 & 0.036 \\
			 
        \bottomrule
	\end{tabularx}
 \vspace{-7pt}
	
\end{table}
